Exact Solutions for Nonlinear Partial Differential Equations: A Fusion of Classical Methods and Innovative Approaches

This article demonstrates how variation of parameters can be successfully implemented in combination with other classical techniques, such as the method of characteristics, to derive novel classes of solutions to nonlinear partial differential equations (NLPDES) by considering specific initial conditions. This innovative approach offers the advantage of generating exact solutions. The results underscore this method's potential to address additional NLPDE classes.

==> references.tex <==
@article{Mahouton,
  title={T. Classes of second order nonlinear differential equations reducible to first order ones by variation of parameters},
 author={M. Hounkonnou Pascal and A. Sielenou},
 journal={arXiv:0902.4175 V1},
 year={2009}
}

@article {D.Zwillinger,
 title={Handbook of Differential Equations},
 author={D. Zwillinger},
 journal={Academic Press, Boston, 3rd edition},
  year={1998}
}

@article{G.M.Murphy,
title={Ordinary Differential Equations and Their Solutions},
 author={G. M. Murphy},
journal={New york},
year={1960}
}

	@inproceedings{Polyanin1,
	title={Handbook of Mathematics for Engineers
		and Scientists}, 
author={A. D. Polyanin and A. V. Manzhirov},
journal={Chapman and Hall/CRC Press, Boca Raton London},
 year={2006} 
}

@article {Polyanin2,
	title={ Handbook of Exact Solutions for Ordinary
		Differential Equations},
author={A. D. Polyanin and A. V. Manzhirov},
journal={Chapman and Hall/CRC Press, Boca Raton, 2nd edition},
	 year={2003} 
}

@article{Panayotounakos,
title={Construction of exact parametric or closed form solutions of some unsolvable classes of nonlinear odes (Abel's nonlinear odes of the first kind and relative degenerate
		equations)},
author={D. E. Panayotounakos and T. I. Zarmpoutis},
journal={International Journal of Mathematics and Mathematical Sciences}, 
 year={2011}
}

@article {Brian,
title={Introduction to the Method of Characteristics},
	author={Brian G Higgins},
 journal={ University of California, Davis CA95616},
 year={2019} 
}

@article {Pozrikidis,
title={ Numerical Computation in Science and Engineering},
author={C. Pozrikidis},
journal={Oxford University Press},
 year={1998}
}

@article {Kamke,
title={Differentialgleichungen: Losungsmethoden und Losungen, I,
		Gewohnliche Differentialgleichungen},
author={E. Kamke},
journal={ B. G. Teubner, Leipzig},
 year={1977}
}

@article {Jovan,
title={ Additions to Kamke's treatise: Variation of parameters
		for nonlinear second order differential equations},
author={Jovan D. Kečkić},
journal={ Univ. Beograd. Pool, Elektrotehn. fak. Ser. Mat. Fiz. No. 544 - No. 576,31-36.},
 year={1946}
}
@article {Boyce,
title={Elementary Differential Equations},
author={W. E. Boyce and R. C. DiPrima},
journal={7th Edition, Wiley, New York},
 year={2000}
}

@article {Zhang,	
title={Doubly periodic solutions of modified Kawahara equation 26, 1155-1160},
	author={D. Zhang}
journal={Chaos,
		Solitons and Fractals, V25, 1155-1160} 
 year={2005}
}
@article {D.Zhang,	
title={New exact travelling wave solutions for some nonlinear evolution equations},
author={D. Zhang},
journal={Chaos,
		Solitons and Fractals, V26, 921-925}, 
 year={2005}
}
@article {Rhee,
title={First-Order Partial Differential Equations},
author={H-K Rhee, R. Aris and N. R. Amundson},
journal={Volume 1, Prentice Hall},
 year={1986}
}

@article {Zachmanoglou,
title={Introduction to Partial Differential Equations with Applications},
author={E. C. Zachmanoglou and D. W. Thoe},
journal={Dover Publications},
year={1986}
}

@article {Kevorkian,
 title={Partial Differential Equations: Analytical Solutions Techniques},
author={J. Kevorkian},
journal={2nd Edition, Springer},
year={1999}
}

@article {Olver,
title={Introduction to Partial Differential Equations},
author={P.J. Olver},
journal={Springer},
year={2014}
}

@article{Myint,
title={ Linear Partial Differential Equations for Scientists and Engineers},
author={U. Myint and L. Debnath},
journal={ 4th Edition. Birkhauser},
year={2007}
}

@article{Hong,
	title={Bäcklund  transformation and n-soliton-like
	solutions to the combined KdV-Burgers equation with variable coefficients},
	author={D. LU, B. Hong and L. Tian},
	journal={International Journal of Nonlinear Science 2, 3-10},
	year={2006}
}

@article{Ablowitz,
	title={Solitons, nonlinear evolution equations and
	inverse scattering transform},
	author={M. J. Ablowitz and P. A. Clarkson},
	journal={Cambridge University Press},
	year={1990}
}
@article{Hong,
	title={Bäcklund  transformation and n-soliton-like
	solutions to the combined KdV-Burgers equation with variable coefficients},
	author={B.Hong and L.Tian},
	journal={International Journal of Nonlinear Science 2, 3-10},
	year={2006}
}

@article{Ablowitz,
	title={Solitons, nonlinear evolution equations and
	inverse scattering transform},
	author={M. J. Ablowitz and P. A. Clarkson},
	journal={Cambridge University Press},
	year={1990}
}
@article{Fan,
	title={Extended tanh-function method and its applications to nonlinear
	equations},
	author={E. Fan},
	journal={Physics Letters A, Volume 277, Issue 4-5, p. 212-218.},
	year={2000}
	doi={10.1016/S0375-9601(00)00725-8}
}
 
 @article{Wazwaz,
 	title={The sine-cosine method for handling nonlinear wave equations},
 	author={A. M. Wazwaz},
 	journal={Math. and Comput. Modeling. 40, (2004) 499-508},
 	year={2004}
 }

  @article{Hassan,
 	title={New Exact Solutions of some (2 + 1)-Dimensional Nonlinear Evolution Equations Via Extended Kudryashov Method},
 	author={M. Hassan, M. Abdel-Razek and H. Shoreh},
 	journal={Reports on Mathematical Physics Volume 74, Issue 3, Pages 347-358 },
 	year={2014}
 	doi={10.1016/S0034-4877(15)60006-4}

 @article{Gana,
 	title={Classes of second order nonlinear partial differential equations reducible to first order},
 	journal={N. Mhadhbi, Gana.S and Alharbi.H. arXiv:2305.03128 },
 	year={2023}

 }
   @article{Kudryashov,
 	title={Extended simplest equation method for nonlinear differential equations},
 	author={N.A. Kudryashov and N.B. Loguinova},
 	journal={Applied Mathematics and Computation.Volume 205, Issue 1, Pages 396-402},
 	year={2008}
 	doi={10.1016/j.amc.2008.08.019}
 }

  @article{Wang,
	title={The (G'/G) expansion method and travelling wave solutions of nonlinear evolution equations in mathematical physics},
	author={M. Wang, X. Li and J. Zhang},
	journal={Physics Letters A. Volume 372, Issue 4, Pages 417-423},
	year={2008}
	doi={10.1016/j.physleta.2007.07.051}
}

 @article{Shikuo,
	title={Jacobi elliptic function expansion method and periodic wave solutions of nonlinear wave equations},
	author={L.Shikuo, F. Zuntao, L. Shida and Z.Qiang},
	journal={Physics Letters A, Volume 289, Issue 1-2, p. 69-74.},
	year={2001}
	doi={10.1016/S0375-9601(01)00580-1}
}
 @article{colostate,
	title={First order partial differential equations:method of characteristics},
	journal={https://mathematics.colostate.edu/}
	
}

@article{Mhadhbi,
title={H. Alharbi. Classes of second order nonlinear partial differential equations reducible to first order},
author={S.Gana, N.Mhadhbi.},
journal={Arxiv.
https://doi.org/10.48550/arXiv.2305.03128 },
year={May.2023}
doi={https://doi.org/10.48550/arXiv.2305.03128}

}

@article{Faddeev,
title={Hamiltonian methods in the theory of
soliton},
author={L. D. Faddeev and L. A. Takhtanjan},
journal={Springer
Series in Soviet Mathematcs. Springer-Verlag, Berlin },
year={1987}

}

@article{Gana1,
title={Pseudospectra of the complex harmonic oscillator},
author={S.Gana and N.Mhadhbi.},
journal={ Global Journal of Pure and Applied Mathematics. Volume 2, number 3 },
year={2007}

}

@article{Gana3,
title={Numerical computation of spectral solutions for Sturm-Liouville Eigenvalue problems},
author={S.Gana},
journal={International Journal of Analysis and Applications},
year={2023}
doi={https://doi.org/10.28924/2291-8639-21-2023-86}
}
@article{Wu,
title={The Variational Iteration Method Which Should be Followed},
author={J. H. He, G. C. Wu and F. Austin,},
journal={Nonlinear Science Letters A. Vol. 1, No. 1, pp. 1-30.},
year={2010}
}

